Exploration by Optimization with Hybrid Regularizers: Logarithmic Regret with Adversarial Robustness in Partial Monitoring

Partial monitoring is a generic framework of online decision-making problems with limited feedback. To make decisions from such limited feedback, it is necessary to find an appropriate distribution for exploration. Recently, a powerful approach for this purpose, \emph{exploration by optimization} (ExO), was proposed, which achieves optimal bounds in adversarial environments with follow-the-regularized-leader for a wide range of online decision-making problems. However, a naive application of ExO in stochastic environments significantly degrades regret bounds. To resolve this issue in locally observable games, we first establish a new framework and analysis for ExO with a hybrid regularizer. This development allows us to significantly improve existing regret bounds of best-of-both-worlds (BOBW) algorithms, which achieves nearly optimal bounds both in stochastic and adversarial environments. In particular, we derive a stochastic regret bound of $O(\sum_{a \neq a^*} k^2 m^2 \log T / \Delta_a)$, where $k$, $m$, and $T$ are the numbers of actions, observations and rounds, $a^*$ is an optimal action, and $\Delta_a$ is the suboptimality gap for action $a$. This bound is roughly $\Theta(k^2 \log T)$ times smaller than existing BOBW bounds. In addition, for globally observable games, we provide a new BOBW algorithm with the first $O(\log T)$ stochastic bound.

==> tex_src/3_ftrl.tex <==
\section{PROPOSED ALGORITHM}\label{sec:ftrl}
This section describes details of the proposed algorithm (Logarithmic Barrier Implicit Normalized Forecaster considering Variances for semi-bandits; \texttt{LBINFV}) by specifying the optimistic prediction $m(t)$, estimator $\hat{\ell}(t)$, and convex regularization $\psi_t$ in~\eqref{eq:defOFTRL}.

We consider two different methods for estimating optimistic predictions; these methods result in regret upper bounds that differ by a constant factor in the stochastic regime and have different data-dependent bounds.
One method is a \emph{least square} (LS) estimation based on the losses thus far, \ie we define $m(t) = (m_1(t), \ldots, m_d(t))^\top \in [0, 1]^d$ by
\begin{align}
  m_i(t) = \frac{1}{1 + N_i(t-1) } \left( \frac{1}{2} + 
  \sum_{s=1}^{t-1} a_i(s) \, \ell_i(s) \right)
  \com 
  \label{eq:defmi_empmean}
\end{align}
where $N_i(t)$ is the number of times the base-arm $i$ is chosen until the $t$-th round, \ie
$N_i(t) = |\{ s \in [t] : a_i(t) = 1 \}|$.
The other method is based on the \emph{gradient descent} (GD), where we define $m(t)$ by 
$m_i(1) = 1/2$ and
\begin{align}
  m_i(t+1)
  =
  \begin{cases}
    (1 - \eta) m_i(t) + \eta \ell_i(t) & \mbox{if} \ i \in I(t)
    \\
    m_i(t) & \mbox{otherwise}    
  \end{cases}
  \label{eq:defmi_grad}
\end{align}
for $i\in[d]$ with a step size $\eta \in (0, 1/2)$.

Let $a(t) \in \calA$ be an action selected at round $t$ and $I(t) = \{i\in[d] : a_i(t) = 1\}$ be the set of base-arms selected at round $t$.
Note that $\{a_i(t) = 1\}$ is equivalent to $\{i \in I(t)\}$ and 
%\begin{align}
$
  \Pr[i \in I(t) | x_i(t)] = \Pr[a_i(t) = 1 | x_i(t)] = x_i(t).
$
%  \per 
%  \n 
%\end{align}

The design of LS is to reduce the leading constant in the regret, and GD is to derive a path-length bound.
LS was developed by~\citet{ito22adversarially}. 
The original idea of GD comes from online learning literature~\citep{herbster2001tracking},
and~\citet{ito2021hybrid} developed the idea in semi-bandits. 
%One can see 
%``key designs that help the later analysis'' can be found in Lemmas 4 \& 5 for LS and Lemma 7 for GD.
%We will add this information in the revised version.
%%(M. Herbster and M. K. Warmuth. Tracking the best linear predictor. JMLR 2001.)

We use an unbiased estimator $\hat{\ell}(t) = ( \hat{\ell}_1(t), \ldots, \hat{\ell}_d(t) )^\top \in \R^d$ of $\ell(t)$ given by
\begin{align}
  \hat{\ell}_i(t) = m_i(t) + \frac{ a_i(t) }{ x_i(t) } (\ell_i(t) - m_i(t)) 
  \label{eq:defellhat}
\end{align}
for $i \in [d]$.
This is indeed an unbiased estimator of ${\ell}(t)$ since
$
\E[ \hat{\ell}_i(t) | x(t) ] 
=
m_i(t) + \frac{x_i(t)}{x_i(t)} (\ell_i(t) - m_i(t))
=
\ell_i(t)
$.
The optimistic prediction $m(t)$ in~\eqref{eq:defellhat} plays a role in reducing the variance of $\hat{\ell}(t)$;
the better $m(t)$ predicts $\ell(t)$,
the smaller the variance in $\hat{\ell}(t)$ becomes.

The regularizer function $\psi_t : \R^d \to \R$ is given by
\begin{align}
%  &
  \psi_t(x) 
  = 
  \sum_{i=1}^d \beta_i(t) \phi (x_i) \com
  \label{eq:defpsi}
\end{align}
where $\phi : \R \to \R$ is defined as
\begin{align}
  \phi(z) = 
  z - 1 - \log z + \gamma \, ( z + (1 - z) \log (1 - z ) )
  \label{eq:defphi}
\end{align}
with $\gamma = \log T$ and regularization parameters $\beta_i(t) \geq 0$.
% \inote{An intuition should be explained.}
Our regularizer in \eqref{eq:defpsi} comprises the logarithmic barrier $- \log x_i$ and
the (negative) Shannon entropy $(1-x_i)\log (1-x_i)$ for the complement of $x_i \in [0,1]$.
Such a regularizer is called a \textit{hybrid} regularizer, and this type of regularizer was employed in existing studies for bounding a component of the regret~\citep{zimmert2019beating, ito22adversarially, ito2022nearly}.
The affine part of the regularizer in~\eqref{eq:defphi}, $z - 1 + \gamma z$, is introduced to simplify the analysis and yields smaller constant factors, which is also used by~\citet{ito22adversarially}.
%\fix{(Q.) any others?}

Regularization parameters $\beta_i(t)$ are defined as 
\begin{align}
%  &
  \beta_i(t) = \sqrt{(1 + \epsilon)^2 + \frac{1}{ \gamma } \sum_{s=1}^{t-1} \alpha_i(s) } 
  \com 
  \label{eq:defalphabeta}
\end{align}
where $\epsilon \in (0, 1/2]$ is an input parameter and
\begin{align}
  \!\!\!
  \alpha_i(t)
  \!=\!
  a_i(t)( \ell_i(t) - m_i(t) )^2 \!\min \!\left\{ 1 ,\frac{2(1 - x_{i}(t))}{x_{i}(t)^2 \gamma} \right\} 
  \per 
  \label{eq:defalpha}
\end{align}
%\new{
%\todo{bimyou?}
We design $\alpha_i(t)$ in~\eqref{eq:defalpha} so that it corresponds to an upper bound of the component of regret, which appears when we use a standard analysis of (O)FTRL with regularizer~\eqref{eq:defpsi}.
We can introduce a $2(1-x_i(t))/(x_i(t)^2 \gamma)$ part in $\alpha_i(t)$ thanks to the Shannon entropy part in regularizer~\eqref{eq:defpsi}.
This part allows us to bound the regret corresponding to optimal base-arms.
The $(\ell_i(t) - m_i(t))^2$ part of $\alpha_i(t)$ comes from the use of optimistic predictions and can be related to the base-arm variances by using the LS and GD methods to estimate $m(t)$.
%}
Algorithm~\ref{alg:lbinfv_semi} summarizes the proposed algorithms.

%\new{
From the intuitive viewpoint, $\alpha_i(t)$ determines the strength of the regularization, and as $\alpha_i(t)$ increases, the algorithm further explores base-arm $i$.
Since $(\ell_i(t) - m_i(t))^2$ in~\eqref{eq:defalpha} represents the squared error of the optimistic prediction, the algorithm becomes more explorative when the loss is unpredictable or has a high variance. 
Also note that $\mu_i \simeq 1$ corresponds to the base-arm with the almost worst expected loss with the least variance. 
The factor $(1-x_i(t))$ in~\eqref{eq:defalpha} contributes to a fast elimination of such a base-arm since the regularization does not become strong when $x_i(t)=1$ is observed.
%}

% ================================
\LinesNumbered
\SetAlgoVlined
\begin{algorithm}[t]
\textbf{input:} action set $\calA$, time horizon $T$

\For{$t = 1, 2, \ldots, T$}{
  Compute $x(t) \in \calX$ by~\eqref{eq:defOFTRL} with $\hat{\ell}(t)$ in~\eqref{eq:defellhat} and $\psi_t$ in~\eqref{eq:defpsi}.
  
  Sample $a(t)$ such that $\E[a(t) | x(t)] = x(t)$.
  
  Take action $a(t)$ and observe feedback $\ell_i(t)$ for $i$ such that $a_i(t) = 1$.
  
  Update the regularization parameters $\beta_i(t)$ in~\eqref{eq:defalphabeta} and optimistic prediction $m_i(t)$ using~\eqref{eq:defmi_empmean} or~\eqref{eq:defmi_grad}.
}
\caption{
\texttt{LBINFV} for semi-bandits
}
\label{alg:lbinfv_semi}
\end{algorithm}
% ================================

% - [what to write]
% - === [on learning rate and regularizer] ===
% - (1 - x) regularization has been used, which is useful for bounding the stability term
% - learning rate alpha is an upper bound of the component & bounded by \sum alpha / beta
% - this is useful to bound the sum over suboptimal basearms (Lemma 6)
% - === [on variance dependence] ===
% - can be linked with variances both with LS and GD estimation of optimistic predictions

%The part of  $2(1-x_i(t))/(x_i(t)^2 \gamma)$ in $\alpha_i(t)$ comes from the Shanon entropy regularizer, 










